backShift: Learning causal cyclic graphs from unknown shift interventions

We propose a simple method to learn linear causal cyclic models in the presence of latent variables. The method relies on equilibrium data of the model recorded under a specific kind of interventions ("shift interventions"). The location and strength of these interventions do not have to be known and can be estimated from the data. Our method, called backShift, only uses second moments of the data and performs simple joint matrix diagonalization, applied to differences between covariance matrices. We give a sufficient and necessary condition for identifiability of the system, which is fulfilled almost surely under some quite general assumptions if and only if there are at least three distinct experimental settings, one of which can be pure observational data. We demonstrate the performance on some simulated data and applications in flow cytometry and financial time series. The code is made available as R-package backShift.

==> add_finance.tex <==
\subsection{Financial time series}
%\begin{table}[h]
%\begin{tabular}{lllll}
%         & DAX    & S\&P 500 & NASDAQ &  \\
%DAX      & 0      & 0.21   & 0.15 &  \\
%S\&P 500 & 1      & 0        & 0.26 &  \\
%NASDAQ   & 0.25 & 0        & 0      & 
%\end{tabular}
%\caption{\ling}
%\end{table}
%
%\begin{table}[h]
%\begin{tabular}{lllll}
%         & DAX    & S\&P 500 & NASDAQ &  \\
%DAX      & 0      & 0.05   & 0.26* &  \\
%S\&P 500 & 3.74*      & 0        & 0 &  \\
%NASDAQ   & 0.13 & 0.10*     & 0      & 
%\end{tabular}
%\caption{\ice}
%\end{table}

\def\arraystretch{1.15}
\begin{figure*}[!tp]
\begin{centering}
%\vspace{-.1cm}
%\hspace{-.65cm}
\subfloat[\ice]
{
    \begin{tabular}{l|llll}
         & DAX    & S\&P 500 & NASDAQ &  \\
         \hline
DAX      & 0      & 0.05   & 0.26* &  \\
S\&P 500 & 3.74*      & 0        & 0 &  \\
NASDAQ   & 0.13 & 0.10*     & 0      & 
\end{tabular}
}
%\hspace{-0.15cm}
\subfloat[\ling]
{
    \begin{tabular}{l|llll}
         & DAX    & S\&P 500 & NASDAQ & \\
         \hline
DAX      & 0      & 0.21   & 0.15 &  \\
S\&P 500 & 1      & 0        & 0.26 &  \\
NASDAQ   & 0.25 & 0        & 0      & 
\end{tabular}
}

%\vspace{-5pt}
\captionof{table}{{\small Point estimates for financial time series data.}}
\end{centering}
\vspace{-5.5mm}
\end{figure*}

==> algo.tex <==
\begin{algorithm}[ht]
\caption{\ice -- Point estimate of connectivity matrix \label{alg:hiddenice}}
	\algorithmicrequire\; Observations: $\X_j \; \forall j \in \J$ %Stability selection parameters: 
  \begin{algorithmic}[1]
  \STATE Compute $\widehat \DSi_{\x,j} \;  \forall j \in \J$
  \STATE $\tilde{\D} = $ { \sc FFDiag}$(\widehat\DSi_{\x,j}) $ 
  \STATE $\hat{\D} = \texttt{PermuteAndScale}(\tilde{\D})$ %$\hat{\D} = \text{diag}(\tilde{\D})^{-1} \cdot \tilde{\D}$
  \STATE$ \hat{\B} = \mb I - \hat{\D}$
  \end{algorithmic}
  \algorithmicensure\; $\hat{\B}$
\end{algorithm} 


==> intervention_vars.tex <==
\subsection{Estimating the intervention variances}\label{sec:Int_vars}
One additional benefit of \ice is that the location and strength of the interventions can be estimated from the data. The empirical, plug-in version of Eq.~\eqref{eq:diff} is given by
\begin{equation}\label{eq:diff_emp}
(\mb I - \hat{\B}) \widehat{\DSi}_{\x,j} (\mb I - \hat{\B})^T = \widehat{\DSi}_{\mb c,j}  = \widehat{\Si}_{\mb c,j} - \widehat{\Si}_{\mb c,-j}\qquad \forall j\in \J.
\end{equation}
So the element $( \widehat{\DSi}_{\mb c,j} )_{kk}$ is an estimate for the difference between the variance of the intervention at variable $k$ in environment $j$ $( \Scj )_{kk}$ and $( \Scjm )_{kk}$. From these differences we can compute the intervention variance for all environments up to an offset, given by the intervention variance in one ``base'' environment we choose. When one of the environments corresponds to observational data, it should be chosen as this base environment since the offset vanishes in this case.
